Modeling Uncertainty Trends for Timely Retrieval in Dynamic RAG

Dynamic retrieval-augmented generation (RAG) allows large language models (LLMs) to fetch external knowledge on demand, offering greater adaptability than static RAG. A central challenge in this setting lies in determining the optimal timing for retrieval. Existing methods often trigger retrieval based on low token-level confidence, which may lead to delayed intervention after errors have already propagated. We introduce Entropy-Trend Constraint (ETC), a training-free method that determines optimal retrieval timing by modeling the dynamics of token-level uncertainty. Specifically, ETC utilizes first- and second-order differences of the entropy sequence to detect emerging uncertainty trends, enabling earlier and more precise retrieval. Experiments on six QA benchmarks with three LLM backbones demonstrate that ETC consistently outperforms strong baselines while reducing retrieval frequency. ETC is particularly effective in domain-specific scenarios, exhibiting robust generalization capabilities. Ablation studies and qualitative analyses further confirm that trend-aware uncertainty modeling yields more effective retrieval timing. The method is plug-and-play, model-agnostic, and readily integrable into existing decoding pipelines. Implementation code is included in the supplementary materials.

==> 1._Intro_old_.tex <==
\section{Introduction}

While large language models(LLMs) achieve remarkable performances on various natural language processing field and significantly transforming the way that human interact with AI-systems~\cite{brown2020language,kaddour2023challenges,bubeck2023sparks,peng2023check,li2023evaluating}, they still face challenges such as limited domain knowledge and outdated training data~\cite{gao2023retrieval,kandpal2023large,mousavi2024your,xiong2024search}. The absence of up-to-date or necessary knowledge often leads to incorrect predictions, undermining the reliability of LLMs in practical scenarios~\cite{maynez2020faithfulness,liu2021token,ji2023survey,peng2023check,}.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{intro}
    \caption{The delayed retrieval issue exists in current dynamic RAG method, where blue tokens represent DRAGIN's retrieval timing, and red tokens highlight incorrectly generated tokens caused by delayed retrieval.}
    \label{pic.intro}
\end{figure}

Retrieval-augmented generation (RAG) has emerged as a popular solution to address the above challenge~\cite{Xu2024UnsupervisedIR,Luo2024LandmarkEA,Fang2024EnhancingNR}. Most existing research focuses on early retrieval during the generation process, aiming to provide external information at the outset to enhance the quality of outputs. However, some research shows that improper retrieval augmentation can negatively influence LLM generation~\cite{ren2023investigating,Ni2024WhenDL,chen2024benchmarking,maekawa2024retrieval} since it may bring redundant or even noisy information. As an alternative, dynamic RAG has been proposed as a more flexible solution, activating retrieval only when necessary. For instance, some works~\cite{borgeaud2022improving,trivedi2022interleaving,ram2023context} perform retrieval after a fixed number of tokens or sentences, while others trigger retrieval when a token's prediction confidence falls below a certain threshold~\cite{jiang2023active,su2024dragin}. 

Although relying on low confidence token for retrieve seems intuitive, we argue that this often results in \textbf{delayed retrieval}, failing to intervene at the optimal moment. Figure~\ref{pic.intro} illustrates several cases where retrieve is triggered when the confidence of a single token falls below a threshold. The results show that when retrieve occurs, the outputs have already deviated from the correct generation path~\footnote{We re-implemented DRAGIN and used the 2WikiMultihopQA~\cite{ho2020constructing} dataset for this analysis.}. This demonstrates that relying on a single token's confidence as the signal can result in ineffective intervention, allowing multiple low-confidence tokens to be generated before retrieve. 

To overcome these limitations, we propose \textbf{E}ntropy-\textbf{T}rend \textbf{C}onstraint (\textbf{ETC}), a novel method that determines retrieval timing based on prediction confidence trends of generated content. ETC measures uncertainty through entropy, but static entropy values alone fail to capture dynamic fluctuations in confidence. Thus we further introduce both first and second differences of the entropy sequence, which are valuable tools for discrete sequence analysis~\cite{jordan1965calculus,levy1992finite,ames2014numerical}. The first difference indicates whether entropy is increasing or decreasing, while the second difference captures the rate of change, making it more sensitive to rapid shifts in confidence. This enables earlier retrieval interventions, preventing the generation of low-confidence tokens  to some extent. However, entropy trend can be affected by outliers, leading to redundant retrieval operations. To mitigate this, we propose a dynamic smoothing technique that stabilizes entropy analysis. By assigning dynamic weights to past generation steps, our method effectively detects significant changes in model uncertainty, ensuring retrieve is triggered at the optimal moment while improving retrieval efficiency.





To verify the effectiveness of our proposed method, we conduct extensive experiments across six commonly used benchmarks with three large language models. The experimental results demonstrate that \textbf{ETC} outperforms various RAG methods while reduces the retrieval count in most cases, particularly when dealing with domain-specific datasets. Besides, we also provide thoroughly ablation studies and in-depth analysis to help readers better understanding our method. The main contributions of this paper are as follows:


\begin{itemize}
    \item We propose a novel \textbf{E}ntropy-\textbf{T}rend \textbf{C}onstraint (\textbf{ETC}) method that incorporates the entropy trend of prediction tokens during the generation process. ETC effectively triggers retrieval before delayed retrieval occurs, enabling external knowledge injection at a more optimal moment.

    \item Experimental results on six widely used datasets with three different LLMs verify the effectiveness of ETC. Besides, we provide extensive in-depth analysis to show the superiority of ETC. The code is available in the supplementary materials. 
\end{itemize}
%We also manually annotate 100 examples and nearly xx\% of them exhibit \textbf{delayed retrieval} problem, as shown in Figure~\ref{fig.intro} (b). 

%, for example, FLARE~\cite{jiang2023active} triggers retrieval dynamically when the LLM’s confidence (i.e., the generation probability) on the next token is lower than certain thresholds, while DRAGIN~\cite{su2024dragin} considers both the generation confidence and the importance of the token


==> checklist.tex <==
\section*{Reproducibility Checklist}

This paper:

\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)

\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)

\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
\end{itemize}

Does this paper make theoretical contributions? (no)

If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)

\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)

\item Proofs of all novel claims are included. (yes/partial/no)

\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)

\item Appropriate citations to theoretical tools used are given. (yes/partial/no)

\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)

\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}


Does this paper rely on one or more datasets? (yes)

If yes, please complete the list below.
\begin{itemize}

\item A motivation is given for why the experiments are conducted on the selected datasets (yes)

\item All novel datasets introduced in this paper are included in a data appendix. (yes)

\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)

\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)

\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)

\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes)

\end{itemize}

Does this paper include computational experiments? (yes)

If yes, please complete the list below.

This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)

Any code required for pre-processing data is included in the appendix. (yes).

All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)

All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)

All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)

If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)

This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)

This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)

This paper states the number of algorithm runs used to compute each reported result. (yes)

Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)

The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)

This paper lists all final 
